Revisiting Learning-based Video Motion Magnification for Real-time Processing

Video motion magnification is a technique to capture and amplify subtle motion in a video that is invisible to the naked eye. The deep learning-based prior work successfully demonstrates the modelling of the motion magnification problem with outstanding quality compared to conventional signal processing-based ones. However, it still lags behind real-time performance, which prevents it from being extended to various online applications. In this paper, we investigate an efficient deep learning-based motion magnification model that runs in real time for full-HD resolution videos. Due to the specified network design of the prior art, i.e. inhomogeneous architecture, the direct application of existing neural architecture search methods is complicated. Instead of automatic search, we carefully investigate the architecture module by module for its role and importance in the motion magnification task. Two key findings are 1) Reducing the spatial resolution of the latent motion representation in the decoder provides a good trade-off between computational efficiency and task quality, and 2) surprisingly, only a single linear layer and a single branch in the encoder are sufficient for the motion magnification task. Based on these findings, we introduce a real-time deep learning-based motion magnification model with4.2X fewer FLOPs and is 2.7X faster than the prior art while maintaining comparable quality.

==> _macros.tex <==
%% PACKAGES (also see cvpr_header.tex)

\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{booktabs}
\usepackage{times}
\usepackage{microtype}
\usepackage{epsfig}
\usepackage[table,xcdraw]{xcolor}
\usepackage{caption}
\usepackage{float}
\usepackage{placeins}
\usepackage{color, colortbl}
\usepackage{stfloats}
\usepackage{enumitem}
\usepackage{tabularx}
\usepackage{xstring}
\usepackage{multirow}
\usepackage{xspace}
\usepackage{url}
\usepackage{subcaption}
\usepackage{xcolor}
\usepackage[hang,flushmargin]{footmisc}
\usepackage{pifont}
\usepackage{transparent}
\usepackage{enumitem}
% Unfortunately, this package interferes with arxiv's stamp
% \ifcamera \usepackage[accsupp]{axessibility} \fi
\usepackage{amsmath}
\usepackage{mathtools}
\usepackage{array}
\usepackage{transparent}
\usepackage{pifont}

% hyperlink
\usepackage[pagebackref,breaklinks,colorlinks,citecolor=blue,linkcolor=blue,bookmarks=false]{hyperref}
\newcounter{tableeqn}[equation]
\renewcommand{\thetableeqn}{\thetable.\arabic{tableeqn}}
\newcounter{tablesubeqn}[tableeqn]
\renewcommand{\thetablesubeqn}{\thetableeqn\alph{tablesubeqn}}

%% MACROS

% \newcommand{\authorname}[1]{{\textcolor{blue}{[Author: #1]}}}
% ...

% \newcommand{\commandname}{string\xspace}
% \definecolor{colorname}{rgb}{0.92,0.49,0.19}

% General

\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

\newcommand{\nbf}[1]{{\noindent \textbf{#1.}}}

\newcommand{\supp}{supplemental material\xspace}
% \ifarxiv \renewcommand{\supp}{appendix\xspace} \fi

\newcommand{\todo}[1]{{\textcolor{red}{[TODO: #1]}}}

% Reviewer commands (1 to 5), e.g. \R{1}, \R{2}
\newcommand{\R}[1]{{%
    \textbf{%
        \ifstrequal{#1}{1}{\textcolor{red}{R#1}}{%
        \ifstrequal{#1}{2}{\textcolor{blue}{R#1}}{%
        \ifstrequal{#1}{3}{\textcolor{magenta}{R#1}}{%
        \ifstrequal{#1}{4}{\textcolor{teal}{R#1}}{%
                           \textcolor{cyan}{R#1}%
        }}}}%
    }%
}}

\newenvironment{packed_enum}{
\begin{enumerate}
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{2pt}
  \setlength{\parsep}{0pt}
}{\end{enumerate}}

\newenvironment{packed_item}{
\begin{itemize}
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{2pt}
  \setlength{\parsep}{0pt}
}{\end{itemize}}


==> figs/tex/noise_sample.tex <==
\begin{figure*}[tp]
    \centering
    \includegraphics[width=0.90\linewidth]{figs/pdf/noise_sample.pdf} \\
    % \vspace{-2mm}
    \caption{\textbf{Magnified outputs and error maps in sub-pixel motion with a noise.} The noise test is conducted with 0.05-pixel small motion and the noise factor of 0.01. The error maps measure the differences between
    % the generated output frame 
    the magnified frames from each method
    and the ground-truth
    magnified
    frame. 
    We 
    % compare the generated 
    generate
    outputs from four methods: (a) Ours, (b) Baseline~\cite{oh2018learning}, (c) Singh~\etal\cite{singh2023lightweight}, and (d) Phase-based method~\cite{wadhwa2013phase}. (c) 
    % Singh~\etal show the similar 
    The error map and magnified frame of Singh~\etal closely resemble to (e) those of input reference frame. 
    % Singh~\etal fail to capture small motion and tend to copy an identical 
    }
    \label{fig:noise_sample}
\end{figure*}

==> figs/tex/noise_test.tex <==
% \renewcommand{\thefigure}{A}
% \begin{figure}[t]
%     \centering
%     \footnotesize
%     \includegraphics[width=0.75\linewidth]{figs/rebuttal/iccv_rebuttal_noise_test.pdf}\\
%     \vspace{-2mm}
%     \caption{\textbf{Quantitative analysis varying spatial resolution.}}
%     \vspace{-6mm}
%     \label{fig:noise}
% \end{figure}

% \renewcommand{\thefigure}{A}
% \setlength{\columnsep}{1mm}%
% \begin{wrapfigure}{r}{0.255\textwidth}
%     \centering
%     \footnotesize
%     \vspace{-4mm}
%     \includegraphics[width=0.255\textwidth]{figs/rebuttal/iccv_rebuttal_noise_test.pdf}\\
%     % \caption{\label{fig:noise}}
%     \vspace{-6mm}
% \end{wrapfigure}
\renewcommand{\thefigure}{A}
\begin{figure}[h]
    \centering
    \footnotesize
    \vspace{-4mm}
    \includegraphics[width=0.98\linewidth]{figs/rebuttal/ss.pdf}
    \vspace{-1.5mm}
    \caption{\textbf{(a) Noise test and (b) Comparison with [40]}}
    \vspace{-5mm}
    \label{fig:noise}
\end{figure}


==> figs/tex/qual.tex <==
\begin{figure}[tp]
    \centering
    \includegraphics[width=.45\textwidth]{figs/pdf/qual.pdf}
    \caption{\textbf{Qualitative comparison on Vanilla Network and Compressed networks}}
    \label{fig:qual}
\end{figure}

==> figs/tex/qual_texture.tex <==
\begin{figure}
    \centering
    \small
    % \includegraphics[width=83mm]{figs/pdf/qual_texture.pdf}
    \includegraphics[width=0.7\linewidth]{figs/pdf/qual_texture.pdf}
    \caption{\textbf{Qualitative analysis for texture preservation.} 
    The magnified frames for the \emph{balance} video clip. In the cropped images, our model is better for texture preservation than the baseline and Singh~\etal~\cite{singh2023lightweight}. 
    The baseline fails to depict textures, which results in blurry pixels.
    Singh~\etal show more blurred results and severe artifacts.
    }
    \label{fig:qual_texture}
\end{figure}

==> figs/tex/scale_indep.tex <==
% \begin{figure*}[t]
%     \centering
%     \small
%         \includegraphics[width=\linewidth]{figs/pdf/scale_indep_v0.pdf}\\
%     (a) spatial resolution (b) decoder channel width (c) decoder layer depth
%     \caption{}
%     \label{fig:scale_indep}
% \end{figure*}

\begin{figure*}[t]
\centering

\resizebox{1\linewidth}{!}{
\small
\begin{tabular}{c c c}
\includegraphics[width=0.33\linewidth]{figs/pdf/scale_indep/scale_indep_spatial_v0.pdf} &
\includegraphics[width=0.33\linewidth]{figs/pdf/scale_indep/scale_indep_ch_v0.pdf} &
\includegraphics[width=0.33\linewidth]{figs/pdf/scale_indep/scale_indep_layer_v0.pdf}\\
(a) Spatial resolution & (b) Decoder channel width & (c) Decoder layer depth \\
\end{tabular}}

% \vspace{2mm}
    \caption{\textbf{Independent scaling results.} Green lines represent the results of baseline variants. Blue lines represent the results of independent scaling on (a) Spatial resolution, (b) Decoder channel width, and (c) Decoder layer depth. 
    }
    % \vspace{-4mm}
    \label{fig:scale_indep}
\end{figure*}

==> figs/tex/spatial_res.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.46\textwidth]{figs/pdf/Figure6_Qualitative_Downsampling.pdf}
    \caption{\textbf{Qualitative results by downsampling.} 
    (Left) We choose two lines in the original frame and (Right) plot a X-T graph for \emph{crane} video. The differences between 
    $2{\times}$ 
    and $4{\times}$ is unnoticeable, 
    in contrast, $8{\times}$ shows more blurry results than 
    $2{\times}$ and 
    $4{\times}$.
    }
    \label{fig:spatial_res}
\end{figure}

==> figs/tex/trend.tex <==
\begin{figure}[tp]
    \centering
    \includegraphics[width=.30\textwidth]{figs/pdf/trend.pdf}
    % \vspace{-2mm}
    \caption{\textbf{Trend line of layer depth and channel dimension.} We independently scale the layer depth $d_D$ and channel dimension $c_D$ and plot the trend line on SSIM and FPS. The slope of the channel dimension is more gradual than the one of the layer depth. 
    % Training is early-stopped at 30 epoch.
    % Higher is better for SSIM.
    }
    \label{fig:trend}
    \vspace{-2mm}
    % \vspace{4mm}
\end{figure}

==> header.tex <==
% 
% \input{_macros}  % Add packages to _macros.tex

%% For cross-referencing labels between documents
\usepackage{xr-hyper}

\makeatletter
\newcommand*{\addFileDependency}[1]{
  \typeout{(#1)}
  \@addtofilelist{#1}
  \IfFileExists{#1}{}{\typeout{No file #1.}}
}

\makeatother
\newcommand*{\myexternaldocument}[1]{
    \externaldocument{#1}
    \addFileDependency{#1.tex}
    \addFileDependency{#1.aux}
}
%%

\usepackage[pagebackref,breaklinks,colorlinks]{hyperref}
% \usepackage[capitalize]{cleveref}
\crefname{section}{Sec.}{Secs.}
\crefname{table}{Table}{Tables}
\crefname{figure}{Fig.}{Figs.}

\frenchspacing

==> tables/ablation_tex_sha.tex <==
% \newcommand\HUGE{\fontsize{60}{72}\selectfont}
% % \renewcommand{\thefigure}{A}
% % \begingroup
% \renewcommand{\arraystretch}{0.9}
% \renewcommand{\thetable}{A}
% \begin{table}[t]
%     \centering
%     \resizebox{1.0\linewidth}{!}{
%         \Huge
%         \begin{tabular}{l c c l l l l}
%         \toprule
%         \multirow{2}[2]{*}{\textbf{Model}} 
%         % & \multirow{2}[2]{*}{\shortstack{Component\\removal}} 
%         & \multirow{2}[2]{*}{\textbf{Shape}} 
%         & \multirow{2}[2]{*}{\textbf{Texture}}
%         & \multirow{2}[2]{*}{\textbf{\#\,Params\,[K]\,$\downarrow$}} 
%         & \multirow{2}[2]{*}{\textbf{FLOPs [G]\,$\downarrow$}} 
%         % & \multirow{2}[2]{*}{\textbf{{\textbf{SSIM} $\uparrow$}}
%         % & \multirow{2}[2]{*}{\textbf{LPIPS} $\downarrow$}}
%         & \multicolumn{2}{c}{\textbf{Quality Metric}}\\
%         \cmidrule(lr){6-7}%
%         & & & & & \multicolumn{1}{l}{\textbf{SSIM} $\uparrow$} & \textbf{LPIPS} $\downarrow$\\
%         \midrule
%         \textbf{[36]} 
%         % & \centering{\transparent{0.5}$-$}
%         & \ding{51}
%         & \ding{51}
%         & 967 & 41.3 & 0.921 & 0.191
%         \\
%         \midrule
%         \multirow{2}{*}{} 
%         % & remove shape
%         & \ding{55}
%         & \ding{51}
%        & 930\,(\blue{-37}) & 39.9\,(\blue{-1.4}) & 0.920\,(\orange{-0.001}) & 0.193\,(\orange{+0.002})
%         \\
%         % & remove texture
%         & \ding{51}
%         & \ding{55}
%         & 930\,(\blue{-37}) & 41.0\,(\blue{-0.3}) & 0.920\,(\orange{-0.001}) & 0.191
%         \\
%         % & remove shape and texture
%         & \ding{55}
%         & \ding{55}
%         & 893\,(\blue{-74}) & 39.6\,(\blue{-1.7}) & 0.921 & 0.191
%         \\
%         \bottomrule
%         \end{tabular}}
%     \vspace{-1mm}
%     \caption{\textbf{Ablation study for texture and shape heads.}}
%     \vspace{-4mm}
%     \label{table:ablation_tex_sha}
% \end{table}

\newcommand\HUGE{\fontsize{60}{72}\selectfont}
% \renewcommand{\thefigure}{A}
% \begingroup
\renewcommand{\arraystretch}{0.9}
\renewcommand{\thetable}{B}
\begin{table}[t]
    \centering
    \resizebox{1.0\linewidth}{!}{
        \Huge
        \begin{tabular}{l c c l l l l}
        \toprule
        \multirow{1}[1]{*}{\textbf{Model}} 
        % & \multirow{2}[2]{*}{\shortstack{Component\\removal}} 
        & \multirow{1}[1]{*}{\textbf{Shape}} 
        & \multirow{1}[1]{*}{\textbf{Texture}}
        & \multirow{1}[1]{*}{\textbf{\#\,Params\,[K]\,$\downarrow$}} 
        & \multirow{1}[1]{*}{\textbf{FLOPs [G]\,$\downarrow$}}
        % & \multirow{2}[2]{*}{\textbf{{\textbf{SSIM} $\uparrow$}}
        % & \multirow{2}[2]{*}{\textbf{LPIPS} $\downarrow$}}
        & \multirow{1}[1]{*}{\textbf{SSIM} $\uparrow$} & \multirow{1}[1]{*}{\textbf{LPIPS}} $\downarrow$\\
        \midrule
        \textbf{[36]} 
        % & \centering{\transparent{0.5}$-$}
        & \ding{51}
        & \ding{51}
        & 967 & 41.3 & 0.921 & 0.191
        \\
        \multirow{2}{*}{} 
        % & remove shape
        & \ding{55}
        & \ding{51}
       & 930\,(\blue{-37}) & 39.9\,(\blue{-1.4}) & 0.920\,(\orange{-0.001}) & 0.193\,(\orange{+0.002})
        \\
        % & remove texture
        & \ding{51}
        & \ding{55}
        & 930\,(\blue{-37}) & 41.0\,(\blue{-0.3}) & 0.920\,(\orange{-0.001}) & 0.191
        \\
        % & remove shape and texture
        & \ding{55}
        & \ding{55}
        & 893\,(\blue{-74}) & 39.6\,(\blue{-1.7}) & 0.921 & 0.191
        \\
        \bottomrule
        \end{tabular}}
    \vspace{-1mm}
    \caption{\textbf{Ablation study for Res.~blocks of shape/texture heads.}}
    \vspace{-7mm}
    \label{table:ablation_tex_sha}
\end{table}

==> tables/architecture.tex <==
\begin{table}[ht]
    \centering
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{c | c c c c c}
        \toprule
        \textbf{Model} & \textbf{$d_D$}& \textbf{$c_D$} & \textbf{Enc. act.}  & \textbf{Enc. Resblocks} & \textbf{Downsampling}\\
        \midrule
         \textbf{Oh~\etal}  & 9 & 64 & Exist & Exist & $2\times$\\
         \textbf{Ours}  & 36 & 32 & None & None & $4\times$ \\
        \bottomrule
        \end{tabular}
    }
    \caption{\textbf{Configurations of architecture of the Oh~\etal~\cite{oh2018learning} and Ours.} $d_D$ denotes the layer depth of the decoder and $c_D$ denotes the channel dimension of the decoder.   }
    \label{table:architecture}
\end{table}

==> tables/architecture_ablation.tex <==
\begin{table}[t]
    \centering
    \resizebox{1.0\linewidth}{!}{
    {\footnotesize
    \centering
        \begin{tabular}{l | c | c c c}
        \toprule
         \textbf{Structural change} & \textbf{FLOPs (G)} $\downarrow$ & \textbf{SSIM} $\uparrow$ &\textbf{LPIPS} $\downarrow$ & \textbf{FPS} $\uparrow$\\
        \midrule
         % $3$  & $112$  & $0.903\,(\orange{-0.018})$ & $0.232\,(\orange{+0.041})$ & $42.3$ \\
         % $6$  & $80$  & $0.915\,(\orange{-0.006})$ & $0.202\,(\orange{+0.011})$ & $42.7$ \\
         Baseline~\cite{oh2018learning}  & $41.3$ & $0.921$ & $0.191$ & $9.6$\\
        %  $12$  & $56$  & $0.923$ & $42.1$ \\
        %  $15$  & $48$  & $0.924$ & $40.0$ \\
         \quad + 1/4~$\times$ Spatial Resolution  & $24.6$ & $0.920$ & $0.203$ & $13.6$ \\
         \quad\quad + Single Linear Encoder & $20.5$ & $0.918$ & $0.208$ & $16.8$\\
         \quad\quad\quad + Scaling $d_D$ and $c_D$  & $9.86$ & $0.918$ & $0.211$ & $25.8$ \\
         \quad\quad\quad\quad + Perceptual Loss (proposed) & $9.86$ & $0.920$ & $0.164$ & $25.8$\\
        \bottomrule
        \end{tabular}
        }
    }
    \vspace{2mm}
\caption{\textbf{Ablation study on structural change in model architecture.} Frames Per Second (FPS) is calculated for input frames of resolution $1920$ $\times$ $1080$.
    % Training is early-stopped at 30 epoch.
    % satisfy the scale $s \simeq s_b$.
    }
    \label{table:compound scaling depth dimension}
    \vspace{-3mm}
\end{table}

 % 0.902\,(\orange{-0.028})
% \begin{table}[ht]
%     \centering
%     \resizebox{0.65\linewidth}{!}{%
%         \begin{tabular}{c c | c c c}
%         \toprule
%          $d_D$ & $w_D$ &\textbf{SSIM} & \textbf{FPS} & \textbf{FLOPs (G)} \\
%         \midrule
%          $3$  & $112$  & $0.903$ & $108.7$ & $42.3$ \\
%          $6$  & $80$  & $0.915$ & $78.1$ & $42.7$ \\
%          $\textbf{9}$  & $\textbf{64}$  & $0.921$ & $83.2$ & $41.3$ \\
%          $12$  & $56$  & $0.923$ & $78.1$ & $42.1$ \\
%          $15$  & $48$  & $0.924$ & $94.2$ & $40.0$ \\
%          $36$  & $32$  & $0.928$ & $85.5$ & $41.5$ \\
%          $144$  & $16$  & $0.925$ & $46.9$ & $41.6$ \\
%         \bottomrule
%         \end{tabular}
%         }
%     \caption{\textbf{Compound factor analysis on layer depth and channel width.} Bold: Vanilla model}
%     \label{table:compound scaling depth width}
% \end{table}


==> tables/channel_total.tex <==
\begin{table}[h]
    \centering
    \resizebox{0.75\linewidth}{!}{%
        \begin{tabular}{c c | c c c}
        \toprule
         \textbf{$w_E$} & \textbf{$w_D$} & \textbf{SSIM} & \textbf{FPS} & \textbf{FLOPs (G)} \\
        \midrule
         $40$  & $80$  & $0.927$ & $51.5$ & $64.2$ \\
         $32$  & $64$  & $0.921$ & $83.2$ & $41.3$ \\
         $24$  & $48$  & $0.912$ & $137.3$ & $23.5$ \\
         $16$  & $32$  & $0.896$ & $201.9$ & $10.6$ \\
         $8$  & $16$  & $0.828$ & $341.2$ & $2.8$ \\
         $4$  & $8$  & $0.793$ & $531.3$ & $0.8$ \\
         % $32$  & $24$  & $0.917$ & $137.4$ & $52.1$ \\
         % $32$  & $16$  & $0.917$ & $137.4$ & $52.1$ \\
         % $32$  & $8$  & $0.917$ & $137.4$ & $52.1$ \\
         
        \bottomrule
        \end{tabular}
    }
    \caption{\textbf{(Left) The table of baseline variants.} \textbf{(Right) The trade-off curve between SSIM and FPS} These results on the table and the trade-off curve are the evaluation results for the models trained by scaling channel width of encoder (Enc.) \textbf{$w_E$} and decoder (Dec.) \textbf{$w_D$} on the baseline model. }
    \label{table:channel_total}
\end{table}

==> tables/collapsing.tex <==
% % \renewcommand{\thefigure}{A}
% \renewcommand{\thetable}{B}

% \begin{table}[t]
%     \centering
%     \renewcommand{\arraystretch}{0.9} 
%     \resizebox{1.0\linewidth}{!}{
%         \large
%         \begin{tabular}{l l l l l}
%         \toprule
%         % \textbf{Model} & \textbf{\# Params\,[K]\,$\downarrow$} & \textbf{FLOPs [G]\,$\downarrow$} & \textbf{SSIM\,$\uparrow$}& \textbf{LPIPS\,$\downarrow$} \\
%         \multirow{2}[2]{*}{\textbf{Model}} 
%         & \multirow{2}[2]{*}{\textbf{\#\,Params\,[K]\,$\downarrow$}} 
%         & \multirow{2}[2]{*}{\textbf{FLOPs [G]\,$\downarrow$}} 
%         & \multicolumn{2}{c}{\textbf{Quality Metric}}\\
%         \cmidrule(lr){4-5}%
%         & & & \multicolumn{1}{l}{\textbf{SSIM} $\uparrow$} & \textbf{LPIPS} $\downarrow$\\
%         \midrule
%          \textbf{Ours} & 716 & 9.05 & 0.917 & 0.172 \\
%          % $+$ applying \emph{Separable} & 709\,(\blue{-7}) & 8.91\,(\blue{-0.14}) & 0.914\,(\orange{-0.003}) & 0.183\,(\orange{+0.011})\\
%           $+$ applying \emph{Collapsing} & 720\,(\orange{+4}) & 8.93\,(\blue{-0.12})& 0.921\,(\blue{+0.04}) & 0.164\,(\blue{-0.008})\\
%         \bottomrule
%         \end{tabular}}
%     \vspace{-1mm}
%     \caption{\textbf{Collapsing three consecutive convolutional layers.}}
%     \vspace{-4mm}
%     \label{table:collapsing}
% \end{table}


% \renewcommand{\thefigure}{A}
\renewcommand{\thetable}{A}

\begin{table}[t]
    \centering
    \renewcommand{\arraystretch}{0.9} 
    \resizebox{1.0\linewidth}{!}{
        \large
        \begin{tabular}{l l l l l}
        \toprule
        % \textbf{Model} & \textbf{\# Params\,[K]\,$\downarrow$} & \textbf{FLOPs [G]\,$\downarrow$} & \textbf{SSIM\,$\uparrow$}& \textbf{LPIPS\,$\downarrow$} \\
        \multirow{1}[1]{*}{\textbf{Model}} 
        & \multirow{1}[1]{*}{\textbf{\#\,Params\,[K]\,$\downarrow$}} 
        & \multirow{1}[1]{*}{\textbf{FLOPs [G]\,$\downarrow$}} 
        & \multirow{1}[1]{*}{\textbf{SSIM} $\uparrow$} & \multirow{1}[1]{*}{\textbf{LPIPS} $\downarrow$}\\
        \midrule
         \textbf{Ours} & 716 & 9.05 & 0.917 & 0.172 \\
         % $+$ applying \emph{Separable} & 709\,(\blue{-7}) & 8.91\,(\blue{-0.14}) & 0.914\,(\orange{-0.003}) & 0.183\,(\orange{+0.011})\\
          $+$ applying \emph{Collapsing} & 720\,(\orange{+4}) & 8.93\,(\blue{-0.12})& 0.921\,(\blue{+0.04}) & 0.164\,(\blue{-0.008})\\
        \bottomrule
        \end{tabular}}
    \vspace{-1mm}
    \caption{\textbf{Collapsing three consecutive convolutional layers.}}
    \vspace{-3.5mm}
    \label{table:collapsing}
\end{table}

==> tables/compound_scaling_depth_dimension.tex <==
\begin{table}[tp]
    \centering
    \resizebox{0.8\linewidth}{!}{
    {\footnotesize
    \centering
        \begin{tabular}{c c | c | c c c}
        \toprule
         $d_D$ & $c_D$ & \textbf{FLOPs (G)} & \textbf{SSIM} $\uparrow$ &\textbf{LPIPS} $\downarrow$ & \textbf{FPS}\\
        \midrule
         % $3$  & $112$  & $0.903\,(\orange{-0.018})$ & $0.232\,(\orange{+0.041})$ & $42.3$ \\
         % $6$  & $80$  & $0.915\,(\orange{-0.006})$ & $0.202\,(\orange{+0.011})$ & $42.7$ \\
         $9$  & $64$ & $41.3$ & $0.921$ & $0.191$ & $83.2$\\
        %  $12$  & $56$  & $0.923$ & $42.1$ \\
        %  $15$  & $48$  & $0.924$ & $40.0$ \\
         $\textbf{36}$  & $\textbf{32}$ & $41.5$ & $\textbf{0.928}$ & $\textbf{0.172}$ & $\textbf{85.5}$ \\
         $144$  & $16$ & $41.6$ & $0.925$ & $0.175$ & $46.9$\\
        \bottomrule
        \end{tabular}
        }
    }
    \vspace{2mm}
\caption{\textbf{Results of jointly scaling layer depth $\boldsymbol{d_D}$ and channel dimension $\boldsymbol{c_D}$.} The configurations of the baseline are $[d_D,c_D]=[9,64]$. Bold: Configurations of the best SSIM, LPIPS, and FPS. Metrics are calculated for input frames of resolution $384 \times 384$.
    % Training is early-stopped at 30 epoch.
    % satisfy the scale $s \simeq s_b$.
    }
    \label{table:compound scaling depth dimension}
    \vspace{-3mm}
\end{table}

 % 0.902\,(\orange{-0.028})
% \begin{table}[ht]
%     \centering
%     \resizebox{0.65\linewidth}{!}{%
%         \begin{tabular}{c c | c c c}
%         \toprule
%          $d_D$ & $w_D$ &\textbf{SSIM} & \textbf{FPS} & \textbf{FLOPs (G)} \\
%         \midrule
%          $3$  & $112$  & $0.903$ & $108.7$ & $42.3$ \\
%          $6$  & $80$  & $0.915$ & $78.1$ & $42.7$ \\
%          $\textbf{9}$  & $\textbf{64}$  & $0.921$ & $83.2$ & $41.3$ \\
%          $12$  & $56$  & $0.923$ & $78.1$ & $42.1$ \\
%          $15$  & $48$  & $0.924$ & $94.2$ & $40.0$ \\
%          $36$  & $32$  & $0.928$ & $85.5$ & $41.5$ \\
%          $144$  & $16$  & $0.925$ & $46.9$ & $41.6$ \\
%         \bottomrule
%         \end{tabular}
%         }
%     \caption{\textbf{Compound factor analysis on layer depth and channel width.} Bold: Vanilla model}
%     \label{table:compound scaling depth width}
% \end{table}


==> tables/computation_time.tex <==
\begin{table}[tp]
    \centering
    \resizebox{0.8\linewidth}{!}{
    {\footnotesize
    \centering
        \begin{tabular}{c | c c c }
        \toprule
        \textbf{Module} & \textbf{Encoder} &\textbf{Manipulator} & \textbf{Decoder}\\
        \midrule
        \textbf{Computation time (\%)} & \textbf{25.7} &\textbf{4.8} & \textbf{69.5}\\
        \bottomrule
        \end{tabular}
        }
    }
    \caption{\textbf{The module-by-module computation time measurement for baseline.
    }}
    \label{table:computation_time_exp}
\end{table}

==> tables/design.tex <==
\begin{table}[t]
    \centering
    \renewcommand{\arraystretch}{1.4} 
    \resizebox{1.0\linewidth}{!}{
        \large
        \begin{tabular}{l l l l l}
        \toprule
        % \textbf{Model} & \textbf{\# Params\,[K]\,$\downarrow$} & \textbf{FLOPs [G]\,$\downarrow$} & \textbf{SSIM\,$\uparrow$}& \textbf{LPIPS\,$\downarrow$} \\
        \multirow{2}[2]{*}{\textbf{Model}} 
        & \multirow{2}[2]{*}{\textbf{\#\,Params\,[K]\,$\downarrow$}} 
        & \multirow{2}[2]{*}{\textbf{FLOPs [G]\,$\downarrow$}} 
        & \multicolumn{2}{c}{\textbf{Quality Metric}}\\
        \cmidrule(lr){4-5}%
        & & & \multicolumn{1}{l}{\textbf{SSIM} $\uparrow$} & \textbf{LPIPS} $\downarrow$\\
        \midrule
         \textbf{Ours} & 716 & 9.05 & 0.917 & 0.172 \\
         $+$ applying \emph{Separable} & 709\,(\blue{-7}) & 8.91\,(\blue{-0.14}) & 0.914\,(\orange{-0.003}) & 0.183\,(\orange{+0.011})\\
          $+$ applying \emph{Merging} & 716 & 8.95\,(\blue{-0.10})& 0.917 & 0.171\,(\blue{-0.001})\\
        \bottomrule
        \end{tabular}}
    \caption{\textbf{Design techniques for more efficient architecture.} Two design techniques are applied to our already established efficient architecture, respectively.
    We substitute the convolutional layers in the encoder with depthwise separable convolution~\cite{monti2018avoiding}, which is denoted as \emph{Seperable}.
    We can also merge adjacent convolutional layers in the encoder into a single layer, which is denoted as \emph{Merging}.
    All the experiments are early-stopped at 30 epochs.
    }
    \label{table:2Yas}
\end{table}


==> tables/dropping.tex <==
\begin{table}[tp]
    \centering
    \caption{\textbf{Experiments with the elimination of Residual block for each module.} We remove the entire Residual Blocks for each module(e.g., Encoder, Manipulator and Decoder).}
    \resizebox{1.0\linewidth}{!}{%
        \begin{tabular}{l c c c c}
        \toprule
        \multirow{2}[2]{*}{Architecture} & \multirow{2}[2]{*}{\#\,params\,[K]} &
        \multirow{2}[2]{*}{FLOPs} &
        \multicolumn{2}{c}{Qualitative metric}\\
        \cmidrule(lr){4-5}
        & & & SSIM & LPIPS\\
        \midrule
        Vanilla\cite{oh2018learning} & 967 & ? & 0.93 & ? \\
        \,- Encoder ResBlock & ? & ? & ? & ? \\
        \,- Manipulator ResBlock & ? & ? & ? & ? \\
        \,- Decoder ResBlock & ? & ? & ? & ? \\
        \bottomrule
        \end{tabular}
    }
    \label{table:drop}
\end{table}



==> tables/generality.tex <==
\begin{table}[tp]
    \centering
    \resizebox{1.0\linewidth}{!}{%
        \begin{tabular}{l c c c}
        \toprule
        \textbf{Model} & \textbf{PSNR [dB]}& \textbf{\# Params} & \textbf{GFLOPs} \\
        \midrule
         \multirow{3}{*}{\textbf{MDSR}} & 35.61 @ 2$\times$ & \multirow{3}{*}{3.23M} & \multirow{3}{*}{@.@@}\\
         & 31.65 @ 3$\times$ & &\\
         & 29.57 @ 4$\times$ & &\\    
         \midrule
         \multirow{3}{*}{\,\,- Head} & 35.61 @ 2$\times$ & \multirow{3}{*}{2.00M} & \multirow{3}{*}{@.@@}\\
         & 31.64 @ 3$\times$ & &\\
         & 29.57 @ 4$\times$ & &\\     
        \bottomrule
        \end{tabular}
    }
    \caption{\textbf{Generalizability}}
    \label{table:generality}
\end{table}


==> tables/preliminary.tex <==
\begin{table}[tp]
    \centering
    \resizebox{1.0\linewidth}{!}{
        {\LARGE
        \begin{tabular}{c  c  c  c}
        \toprule
        \textbf{Module} & \textbf{Input} & \textbf{Network Components} & \textbf{Output}\\
        \midrule
        (a) Enc. 
        & $[ H, W, 3 ]$ 
        & Conv$\times$ 2, Resblk$\times$ 3, (d), (e) 
        & See (d), (e)\\
        (b) Man. 
        & $[ H/2, W/2, 32 ]$
        & Conv$\times$ 2, Resblk$\times$ 1 
        & $[ H/2, W/2, 32 ]$\\
        (c) Dec. 
        & $[ H/2, W/2, 64 ]$
        & Conv$\times$ 2, Resblk$\times$ 9  
        & $[ H, W, 3 ]$\\
        \midrule
        (d) Shape header 
        & $[ H/2, W/2, 32 ]$ 
        & Conv$\times$ 1, Resblk$\times$ 2 
        & $[ H/2, W/2, 32 ]$\\
        (e) Texture header 
        & $[ H/2, W/2, 32 ]$ 
        & Conv$\times$ 1, Resblk$\times$ 2  
        & $[ H/4, W/4, 32 ]$\\
        \bottomrule
        \end{tabular}}
    }
     \caption{Details of modules of the baseline model.}
    \label{table:preliminary}
\end{table}

==> tables/removal_exp_sup.tex <==
\begin{table*}[t]
    \centering
    \caption{\textbf{Experiments with the component removal in residual blocks for each module.} We induce a generalized form of function using learnable parameter and take out ReLU, skip-connection of residual block, and even whole residual block for each module(e.g., the encoder, the manipulator, and the decoder). There are total 17 Residual blocks. First 7 blocks depict the encoder residual blocks. We represent these 7 blocks sequentially as 3 common blocks shared by Frame A and B, 2 texture header blocks, and 2 shape header blocks. One in the middle represents the block in the manipulator. The last 9 ones represent the blocks of the decoder. We describe the removed components as dotted line, remaining as gray, and non-parametric (i.e., same as baseline) as slash pattern.} 
    \resizebox{1.0\linewidth}{!}{
        {\LARGE
        \begin{tabular}{c l c c c c c c c c}
        \toprule
        \multirow{2}[2]{*}{\shortstack{Parametric\\removal}} 
        & \multirow{2}[2]{*}{Module} 
        & \multicolumn{2}{c}{Non-linearity} 
        & \multirow{2}[2]{*}{Conv. layer} 
        & \multirow{2}[2]{*}{Removed (dotted), remaining (gray), and non-parameterized (slash) blocks.} 
        & \multirow{2}[2]{*}{\#\,params\,[K]} 
        & \multirow{2}[2]{*}{FLOPs} 
        & \multicolumn{2}{c}{Qualitative metric}\\
        \cmidrule(lr){3-4} \cmidrule(lr){9-10}%
        && ReLU & Skip & & & & & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
        \midrule
        $-$ 
        & Baseline~\cite{oh2018learning} 
        & \ding{51} 
        & \ding{51} 
        & \ding{51} 
        & \vcenter{\includegraphics[width=1.0\textwidth]{figs/pdf/table1/table1_vanilla.pdf}} 
        & 967 & 41.32 & 0.93 & 0.19
        \\
        \midrule
        \multirow{4}[4]{*}{Deactivation} 
        & Encoder 
        & \multirow{4}[4]{*}{\transparent{0.2}{\ding{55}}} 
        & \multirow{4}[4]{*}{\ding{51}} 
        & \multirow{4}[4]{*}{\ding{51}} 
        & \vspace{3mm}\vcenter{\includegraphics[width=1.0\textwidth]{figs/pdf/table1/table1_enc_dot.pdf}} 
        & 967 & 41.308 & 0.9287 & 0.1871
        \\
        & Manipulator 
        & & & 
        & \vspace{3mm}\vcenter{\includegraphics[width=1\textwidth]{figs/pdf/table1/table1_man_dot.pdf}} 
        & 967 & 41.314 & 0.9298 & 0.1814
        \\
        & Decoder 
        & & & 
        & \vspace{1mm}\vcenter{\includegraphics[width=1\textwidth]{figs/pdf/table1/table1_dec_deact_dot.pdf}} 
        & 967 & 41.30 & 0.9017 & 0.2527
        \\
        & \quad w/ coercive removal 
        & & & 
        & \vcenter{\includegraphics[width=1\textwidth]{figs/pdf/table1/table1_dec_coercive.pdf}} 
        & 967 & 41.29 & 0.8307 & 0.3367
        \\
        \midrule
        \multirow{4}[4]{*}{Disconnection} 
        & Encoder 
        & \multirow{4}[4]{*}{\ding{51}} 
        & \multirow{4}[4]{*}{\transparent{0.2}{\ding{55}}} 
        & \multirow{4}[4]{*}{\ding{51}} 
        & \vspace{3mm}\vcenter{\includegraphics[width=1\textwidth]{figs/pdf/table1/table1_enc_dot.pdf}} 
        & 967 & ? & ? & ?
        \\
        & Manipulator 
        & & & 
        & \vspace{3mm}\vcenter{\includegraphics[width=1\textwidth]{figs/pdf/table1/table1_man_dot.pdf}} 
        & 967 & ? & ? & ?
        \\
        & Decoder 
        & & & 
        & \vspace{1mm}\vcenter{\includegraphics[width=1\textwidth]{figs/pdf/table1/table1_dec_skip_dot.pdf}} 
        & 967 & ? & ? & ?
        \\
        & \quad w/ coercive removal 
        & & & 
        &  \vcenter{\includegraphics[width=1\textwidth]{figs/pdf/table1/table1_dec_coercive.pdf}} 
        & 967 & 41.315 & ? & ?
        \\
        \midrule
        \multirow{4}[4]{*}{Dropping out} & Encoder & \multirow{4}[4]{*}{\transparent{0.2}{\ding{55}}} & \multirow{4}[4]{*}{\transparent{0.2}{\ding{55}}} & \multirow{4}[4]{*}{\transparent{0.2}{\ding{55}}} & \vspace{3mm}\vcenter{\includegraphics[width=1\textwidth]{figs/pdf/table1/table1_enc_dot.pdf}} 
        & 838 & 37.56 & 0.9284 & 0.1863
        \\
        & Manipulator 
        & & & 
        & \vspace{3mm}\vcenter{\includegraphics[width=1\textwidth]{figs/pdf/table1/table1_man_dot.pdf}} 
        & 948 & 40.63 & 0.9296 & 0.1822
        \\
        & Decoder 
        & & & 
        & \vspace{1mm}\vcenter{\includegraphics[width=1\textwidth]{figs/pdf/table1/table1_dec_drop_dot.pdf}} 
        & 524 & 24.97 & 0.8635 & 0.3167
        \\
        &\quad$\vdash$ w/ coercive removal 
        & & & 
        & \vcenter{\includegraphics[width=1\textwidth]{figs/pdf/table1/table1_dec_coercive.pdf}} 
        & 302 & 16.79 & 0.8525 & 0.3299 
        \\
        \bottomrule
        \end{tabular}
        }
    }
    \label{table:nonlinear}
\end{table*}

==> tables/removal_function.tex <==
% \begin{table}[h]
%     \centering
%     \resizebox{1.0\linewidth}{!}{%
%         {\LARGE
%         \def\arraystretch{1.5}
%         \begin{tabularx}\textwidth{@{}lML@{}}
%         \toprule
%         \textbf{Neural components} & \multicolumn{1}{l}{\textbf{Definition}}
%                                   & \multicolumn{1}{r}{} & \multicolumn{1}{r}{}\\ \midrule
%         Non-linear activation & \multicolumn{1}{l}{\textbf{$f(x) = (1-\alpha)\sigma(x) + \alpha x$}}
%                         & eq:act_func \\
%         Skip connection & \multicolumn{1}{l}{\textbf{$f(x) = (1-\beta)G(x) + \beta (G(x)-x)$}}
%                         & eq:skip_func \\
%         Residual block     & \multicolumn{1}{l}{\textbf{$f(x) = (1-\gamma)G(x) + \gamma x$}}
%                         & eq:block_func \\
%         \bottomrule
%         \end{tabularx}}
%     }
%     \label{table:removal_func}
% \end{table}

\begin{table}[tp]\centering
\resizebox{1.0\linewidth}{!}{%
{\LARGE
\def\arraystretch{1.3}
\begin{tabular}{llr}
\toprule
\multirow{1}[1]{*}{\textbf{Neural component}} & \multirow{1}[1]{*}{\textbf{Definition}} & \multirow{1}[1]{*}{}\\
\midrule
Non-linear activation & $f(x) = (1-\omega)\sigma(x) + \omega x$ &\\
% \begin{equation}
% \end{equation}
% \label{eq:act_func}\\
Skip connection & $f(x) = (1-\omega)G(x) + \omega (G(x)-x)$ &\\
% \begin{equation}
% \end{equation}
% \label{eq:skip_func}\\
Residual block & $f(x) = (1-\omega)G(x) + \omega x$ &\\
% \begin{equation}
% \end{equation}
% \label{eq:block_func}\\
\bottomrule
\end{tabular}}}
\caption{Removal function for each component}\label{table:removal_func}\end{table}
